Measuring Conversational Uptake: A Case Study on Student-Teacher Interactions

In conversation, uptake happens when a speaker builds on the contribution of their interlocutor by, for example, acknowledging, repeating or reformulating what they have said. In education, teachers' uptake of student contributions has been linked to higher student achievement. Yet measuring and improving teachers' uptake at scale is challenging, as existing methods require expensive annotation by experts. We propose a framework for computationally measuring uptake, by (1) releasing a dataset of student-teacher exchanges extracted from US math classroom transcripts annotated for uptake by experts; (2) formalizing uptake as pointwise Jensen-Shannon Divergence (pJSD), estimated via next utterance classification; (3) conducting a linguistically-motivated comparison of different unsupervised measures and (4) correlating these measures with educational outcomes. We find that although repetition captures a significant part of uptake, pJSD outperforms repetition-based baselines, as it is capable of identifying a wider range of uptake phenomena like question answering and reformulation. We apply our uptake measure to three different educational datasets with outcome indicators. Unlike baseline measures, pJSD correlates significantly with instruction quality in all three, providing evidence for its generalizability and for its potential to serve as an automated professional development tool for teachers.

==> scratch.tex <==

\section{Linguistic Analysis}


\begin{figure}[]
 \centering
   \centering
  \includegraphics[width=\linewidth]{plots/speech_acts.png}
   \caption{Switchboard speech acts and uptake}
   \label{fig:speech_acts}
\end{figure}

\paragraph{Mirroring.}

\paragraph{Question-answering.}

\paragraph{Use of ``you''.}

\paragraph{Cognition words.}

%Our proposed uptake model, which we describe in Section~\ref{sec:uptake_model} is based on next utterance classification (henceforth, \nuc). For this model, we fine-tune a pre-trained Bert-base model \citep{devlin2019bert} for one epoch on all examples with a batch size of 32, with a maximum length of 120 tokens for each sequence $s$ and $t$ within an $(s,t)$ pair. For optimization, we use Adam with a learning rate of 6.25e-5. We use linear learning rate decay and a dropout probability of $.1$ on all layers. Training took approximately 1.5hrs on a single TitanX GPU.



%\paragraph{Label propagation.} Label propagation has proven to be an effective classification approach in instances with limited amount of labeled data \citep{speriosu2011twitter,hamilton2016inducing}. Inspired by this work, we also experiment with a few-shot approach combined with label propagation (\lprop), where we randomly select 10 examples labeled by at least two raters for having high uptake (high-set) and 10 examples labeled by at least two raters for having low uptake (low-set). Then, we compute the average pairwise similarities $sim_{high}$ and $sim_{low}$ of all other examples to each example in the high-set and the low-set, respectively. We estimate utterance similarities using the \usim{} approach described above. Finally, we obtain uptake labels by computing the ratio $sim_{high} / sim_{low}$.

%\paragraph{Traditional supervision.} As the final baseline, we consider a standard supervised approach (\supervised), which is \emph{not} an available option in most instances due to resource constraints and/or data privacy reasons (Section~\ref{sec:intro}). For this baseline, we fine-tune Bert-base via 5-fold cross-validation using a regression task. \todo{add parameters}




\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|}
\hline
\textbf{Example}                                                                                                                                                                                                                                                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}}\textbf{Human label} \end{tabular}   & \begin{tabular}[c]{@{}l@{}}\textbf{Model Score} \end{tabular}    \\ \hline
\begin{tabular}[c]{@{}l@{}}$S$: You would multiply 4 times 3 and then add 1.\\ $T$: So if I multiply 4 times 3, what does that give me? \end{tabular}                                                                                                                                                                                                                                                   & high                      & \multirow{3}{*}{top 25\%}    \\ \cline{1-2}
\begin{tabular}[c]{@{}l@{}}$S$: I don't think it's any of those.  I think it's between 10 and 100 because I know that 7 times\\ 12 is 84, and 84 is less than ––\\ $T$: Because 7 times 12 –– you're saying if I thought about this as 84 divided by 7, that's equal to 12?"\end{tabular}                                                                                                              & high                      &                              \\ \cline{1-2}
\begin{tabular}[c]{@{}l@{}}$S$: You have to – if it’s an improper fraction—\\ $T$: Very good.  Bring that up.  If it’s a what?\end{tabular}                                                                                                                                                                                                                                                            & high                      &                              \\ \hline \hline
\begin{tabular}[c]{@{}l@{}}$S$: Oh yeah I thought it was 14 by 2.\\ $T$: 14 by 1 thank you Student C. 14 plus 14 is 28. 28 plus 2. The reason why I said that is because\\ I have 1 here and 1 here 14 plus 2.\end{tabular}                                                                                                                                                                            & mid                       & \multirow{3}{*}{middle 25\%} \\ \cline{1-2}
\begin{tabular}[c]{@{}l@{}}$S$: They're all gonna be acute.\\ $T$: All gonna be acute.  Excellent.  All gonna be acute.  So let's do this.  We're out of time. But let's do \\this real quick. I wanna show you how to cut these triangles out.  Let's just cut out the top ones real quick. \\ Just cut out the top ones.   And don't cut out the actual triangle, cut out the squares.\end{tabular} & mid                       &                              \\ \cline{1-2}
\begin{tabular}[c]{@{}l@{}}$S$: Teacher, how do you get 15?\\ T: Take a look.  Take a look.  All right, you're in-between.\end{tabular}                                                                                                                                                                                                                                                              & mid                       &                              \\ \hline \hline
\begin{tabular}[c]{@{}l@{}}$S$: She said she wants to—\\ $T$: Work on this one then.\end{tabular}                                                                                                                                                                                                                                                                                                      & low                       & \multirow{3}{*}{bottom 25\%} \\ \cline{1-2}
\begin{tabular}[c]{@{}l@{}}$S$: I added the three holes and then I used the fours and added it to the one eighth.\\ $T$: Who can explain that to me a little more clearly?\end{tabular}                                                                                                                                                                                                                & low                       &                              \\ \cline{1-2}
\begin{tabular}[c]{@{}l@{}}$S$: You have to find a multiple of the two denominators.\\$T$: Uh-huh.  So remember when we just worked with fractions and not whole numbers?\end{tabular}                                                                                                                                                                                                                & low                       &                              \\ \hline
\end{tabular}
}
\caption{Example exchanges between the teacher and the student.}
\label{tab:math_examples}
\end{table*}


To compare the models' predictions with the human labels, we turn human labels into numerical scores (``low'': 0, ``mid'': 1, ``high'': 2). We compute the Spearman rank order correlation between the models' predictions and the human labels averaged across the three raters -- the results are shown in Table~\ref{tab:results}.

%We find that our estimates of PPMI and JSD both have a highly significant correlation with the human labels. Our best model is PPMI w/ maskrep, which has a correlation of .68 ($p < .001$) with the human labels. JSD w/ maskrep also has a highly significant correlation of .59 ($p<.001$) with human labels. We find that masking repetition provides a significant boost in the case of both PPMI and JSD (add significance).  \todo{use z-scoring to compute the significance of the difference between correlations}


%The results support our information theoretic model of uptake (Section~\ref{sec:uptake_model}), as a function of two components: relevance and informativeness. In particular, PPMI correlates significantly better with the human labels than the two individual sub-components of PPMI, $p(T)$ $p(T|S)$. As we expected, $p(T)$ shows a significant negative correlation with the human labels (-.33), suggesting that uptake increases with the uniqueness ($\sim$informativeness), of $T$. However, the correlation of $p(T)$ with human judgments is significantly lower than that of PPMI \todo{add significance}. Interestingly, $p(T|S)$ does not correlate significantly with human labels, suggesting that without controlling for $p(T)$, conditional probability is not a reliable measure of uptake.

%Among the baseline models, the word overlap model is the only one with a significant correlation with the human labels (), but even that correlation is significantly lower than the correlation among PPMI and JSD and the human labels (\todo{add significance}). The fact that word overlap correlates with human labels is expected, given that this measure also incorporates a notion of informativeness (word overlap increases with the number of words) and relevance (approximated by overlap). However, as we discussed in Section~\ref{sec:uptake_definition}, uptake is more than just repetition. The fact that word overlap is not as good at estimating uptake as PPMI and JSD suggest that our model \emph{does} pick up on salient aspects of uptake beyond repetition.

%\paragraph{Examples and error analysis.} Table~\ref{tab:math_examples} shows a sample of examples annotated by the 

